Towards Energy Efficient Mobile Eye Tracking for AR Glasses through Optical Sensor Technology

After the introduction of smartphones and smartwatches, AR glasses are considered the next breakthrough in the field of wearables. While the transition from smartphones to smartwatches was based mainly on established display technologies, the display technology of AR glasses presents a technological challenge. Many display technologies, such as retina projectors, are based on continuous adaptive control of the display based on the user's pupil position. Furthermore, head-mounted systems require an adaptation and extension of established interaction concepts to provide the user with an immersive experience. Eye-tracking is a crucial technology to help AR glasses achieve a breakthrough through optimized display technology and gaze-based interaction concepts. Available eye-tracking technologies, such as VOG, do not meet the requirements of AR glasses, especially regarding power consumption, robustness, and integrability. To further overcome these limitations and push mobile eye-tracking for AR glasses forward, novel laser-based eye-tracking sensor technologies are researched in this thesis. The thesis contributes to a significant scientific advancement towards energy-efficient mobile eye-tracking for AR glasses.

==> head/dedication.tex <==
\cleardoublepage
\thispagestyle{empty}


\vspace*{3cm}

\begin{raggedleft}
    	Wings are a constraint that makes \\
	it possible to fly.\\
     --- Robert Bringhurst\\
\end{raggedleft}

\vspace{4cm}

\begin{center}
    To my parents\dots
\end{center}




==> tail/A2/bibliography.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{a1.png}}]{First A. Author} (M'76--SM'81--F'87) and all authors may include 
biographies. Biographies are often not included in conference-related
papers. This author became a Member (M) of IEEE in 1976, a Senior
Member (SM) in 1981, and a Fellow (F) in 1987. The first paragraph may
contain a place and/or date of birth (list place, then date). Next,
the author's educational background is listed. The degrees should be
listed with type of degree in what field, which institution, city,
state, and country, and year the degree was earned. The author's major
field of study should be lower-cased. 

The second paragraph uses the pronoun of the person (he or she) and not the 
author's last name. It lists military and work experience, including summer 
and fellowship jobs. Job titles are capitalized. The current job must have a 
location; previous positions may be listed 
without one. Information concerning previous publications may be included. 
Try not to list more than three books or published articles. The format for 
listing publishers of a book within the biography is: title of book 
(publisher name, year) similar to a reference. Current and previous research 
interests end the paragraph. The third paragraph begins with the author's 
title and last name (e.g., Dr.\ Smith, Prof.\ Jones, Mr.\ Kajor, Ms.\ Hunter). 
List any memberships in professional societies other than the IEEE. Finally, 
list any awards and work for IEEE committees and publications. If a 
photograph is provided, it should be of good quality, and 
professional-looking. Following are two examples of an author's biography.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{a2.png}}]{Second B. Author} was born in Greenwich Village, New York, NY, USA in 
1977. He received the B.S. and M.S. degrees in aerospace engineering from 
the University of Virginia, Charlottesville, in 2001 and the Ph.D. degree in 
mechanical engineering from Drexel University, Philadelphia, PA, in 2008.

From 2001 to 2004, he was a Research Assistant with the Princeton Plasma 
Physics Laboratory. Since 2009, he has been an Assistant Professor with the 
Mechanical Engineering Department, Texas A{\&}M University, College Station. 
He is the author of three books, more than 150 articles, and more than 70 
inventions. His research interests include high-pressure and high-density 
nonthermal plasma discharge processes and applications, microscale plasma 
discharges, discharges in liquids, spectroscopic diagnostics, plasma 
propulsion, and innovation plasma applications. He is an Associate Editor of 
the journal \emph{Earth, Moon, Planets}, and holds two patents. 

Dr. Author was a recipient of the International Association of Geomagnetism 
and Aeronomy Young Scientist Award for Excellence in 2008, and the IEEE 
Electromagnetic Compatibility Society Best Symposium Paper Award in 2011. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{a3.png}}]{Third C. Author, Jr.} (M'87) received the B.S. degree in mechanical 
engineering from National Chung Cheng University, Chiayi, Taiwan, in 2004 
and the M.S. degree in mechanical engineering from National Tsing Hua 
University, Hsinchu, Taiwan, in 2006. He is currently pursuing the Ph.D. 
degree in mechanical engineering at Texas A{\&}M University, College 
Station, TX, USA.

From 2008 to 2009, he was a Research Assistant with the Institute of 
Physics, Academia Sinica, Tapei, Taiwan. His research interest includes the 
development of surface processing and biological/medical treatment 
techniques using nonthermal atmospheric pressure plasmas, fundamental study 
of plasma sources, and fabrication of micro- or nanostructured surfaces. 

Mr. Author's awards and honors include the Frew Fellowship (Australian 
Academy of Science), the I. I. Rabi Prize (APS), the European Frequency and 
Time Forum Award, the Carl Zeiss Research Award, the William F. Meggers 
Award and the Adolph Lomb Medal (OSA).
\end{IEEEbiography}

==> tail/D1/New_Evaluation.tex <==
\section{Evaluation}
\label{Evaluation}


\subsection{LFI sensor noise characterization}
\begin{figure}
	\centering
 	\includegraphics[width=\linewidth]{Images/Characterization.pdf}	
	\caption{tbd.}
	\label{fig:sensor_charac}
\end{figure}

- Labsetup von Mario mit einem Sensor 


- Distanz- und Geschwindigkeitsrauschen über Messbereich

\subsection{Part of the eye classifier accuracy}

- Rauschen beschreiben
\input{Images/tikz/classifierResult.tikz}

\input{Images/tikz/classifierResultMuSigma.tikz}

- Schätzung der Sensorpositionen -> Wie lange dauert es bis Sensorpositionen konvergieren für 20 Part. ? 


- Surrogat model rekonstruktion (Kartoffel und Iris scheibe)


- Blickwinkelschätzung

\subsection{Glasses slippage compensation}

\begin{figure}
	\centering
	\input{Images/tikz/sensorPositionEstimationSimulation.tikz}	
	\caption{Estimated translation between head-fixed and glasses-fixed coordinates.}
	\label{fig:sensorPositionEstimationSimulation}
\end{figure}


\subsection{Gaze estimation}

- Abb. der verwendeten Geometrie (Sensorpositionen)




- Abb. der verwendeten Augen Trajektorie

\begin{figure}
	\centering
	\input{Images/tikz/eyeRefTrajectory.tikz}	
	\caption{Reference eye trajectory.}
	\label{fig:eyeRefTrajectory}
\end{figure}

\begin{figure}
	\centering
	\input{Images/tikz/gazeEstimationSimulation.tikz}	
	\caption{Simulation result: Gaze estimation (w/ and w/o offset compensation), estimation error.}
	\label{fig:gazeEstimationSimulation}
\end{figure}


%\subsubsection{Gaze angle estimation accuracy with artificial data}
% Ich glaube, wir brauchen diese eytra Subsubsection nicht - wenn es direkt auch mit slippage geht und die Methode dafür nicht anders ist, können wir auch direkt das coolere Szenario zeigen



%\subsection{Gaze angle estimation accuracy and glasses slippage}
%- Schätzung der Sensorpositionen (nur Translation, rotation vernachlässigbar)
%
%
%- Surrogat model rekonstruktion (Kartoffel und Iris scheibe)
%
%
%- Blickwinkelschätzung
%
%
%
%
%
%\subsubsection{Gaze angle estimation accuracy with real trajectory}
%- Pupil labs aufzeichnung als input über längeren zeitraum 










%\subsection{Laboratory results}
%- Laboraufbau beschreiben (Taucherbrille mit 4 LFI sensoren) + Kamera
%
%
%- Eye safety
%
%
%- Experimentdesign -> nacheinander 13 Punkte auf Monitor anschauen
%
%
%\subsection{Part of the eye classifier accuracy}
%
%\subsubsection{Gaze angle estimation accuracy}

==> tail/D1/definitions.tex <==
\tikzset{
 int/.style={
  draw=black,
  minimum size=8mm,
  alias=thisone,
  append after command={(thisone.south west) -- (thisone.north east)}
 }
}

\tikzstyle{sum} = [circle,draw,minimum size=2mm,inner sep=0pt]

\definecolor{boschred}{RGB}{215,0,18}
\definecolor{fuchsia}{RGB}{168,1,99}
\definecolor{violet}{RGB}{63,19,108}
\definecolor{darkblue}{RGB}{8,66,126}
\definecolor{lightblue}{RGB}{14,120,197}
\definecolor{blueAkzent3}{RGB}{184,217,251}
\definecolor{blueAkzent4}{RGB}{199,229,251}
\definecolor{lightblue}{RGB}{14,120,197}
\definecolor{turquoise}{RGB}{19,153,160}
\definecolor{lightgreen}{RGB}{103,180,25}
\definecolor{darkgreen}{RGB}{10,81,57}
\definecolor{darkgray}{RGB}{66,76,88}
\definecolor{lightgray}{RGB}{178,179,181}

\definecolor{matlab1}{rgb}{0,    	  0.4470,    0.7410}
\definecolor{matlab2}{rgb}{0.8500,    0.3250,    0.0980}
\definecolor{matlab3}{rgb}{0.9290,    0.6940,    0.1250}
\definecolor{matlab4}{rgb}{0.4940,    0.1840,    0.5560}
\definecolor{matlab5}{rgb}{0.4660,    0.6740,    0.1880}
\definecolor{matlab6}{rgb}{0.3010,    0.7450,    0.9330}
\definecolor{matlab7}{rgb}{0.6350,    0.0780,    0.1840}



\pgfdeclarelayer{background}
\pgfsetlayers{background,main}

\newcommand{\figref}[1]{Fig.~\ref{#1}}
%\newcommand{\algref}[1]{Alg.~\ref{#1}}

\newcommand{\Ts}{T_\text{s}}
\newcommand{\npdf}[3]{\mathcal{N}\! \left(#1 \, \left| \, #2, #3 \right. \right)}
\newcommand{\condProb}[2]{p\! \left(#1  \, \left| \, #2\right. \right)}
\newcommand{\bE}[2]{\mathbb{E}_{#1}\left[#2\right]}
\newcommand{\Qfun}[2]{\mathcal{Q}\! \left(#1 , #2 \right)}
\newcommand{\gfun}[1]{\gamma\! \left(#1 \right)}
\newcommand{\zk}[1]{z_{#1}(k)}
\newcommand{\zkm}[1]{z_{#1}(k-1)}

\newcommand{\xg}{x_{\text{g}}}
\newcommand{\sg}{s_{\text{g}}}
\newcommand{\xh}{x_{\text{h}}}
\newcommand{\yh}{y_{\text{h}}}
\newcommand{\sh}{s_{\text{h}}}
\newcommand{\xe}{x_{\text{e}}}
\newcommand{\se}{s_{\text{e}}}

\newcommand{\xgi}{x_{\text{g},i}}
\newcommand{\sgi}{s_{\text{g},i}}
\newcommand{\xhi}{x_{\text{h},i}}
\newcommand{\shi}{s_{\text{h},i}}
\newcommand{\xei}{x_{\text{e},i}}

\newcommand{\bR}{\mathbb{R}}
\newcommand{\Ns}{N_\text{s}}

\newcommand{\rsc}{r_\text{sclera}}
\newcommand{\rrt}{r_\text{retina}}

\newcommand{\dt}{\; d \text{t}}
\newcommand{\diris}{d_\text{iris}}
\newcommand{\niris}{n_\text{iris}}
\newcommand{\nirisx}{n_{\text{iris},x}}
\newcommand{\nirisy}{n_{\text{iris},y}}
\newcommand{\nirisz}{n_{\text{iris},z}}


==> tail/cv.tex <==
\cleardoublepage
\thispagestyle{empty}
\phantomsection
\addcontentsline{toc}{chapter}{Curriculum Vitae}
\ifpdf
\includepdf[pagecommand=\thispagestyle{addpagenumbersforpdfimports},pages=-]{tail/cv.pdf}
\fi
